A multi-paradigm language for reactive synthesis

This paper proposes a language for describing reactive synthesis problems that integrates imperative and declarative elements. The semantics is defined in terms of two-player turn-based infinite games with full information. Currently, synthesis tools accept linear temporal logic (LTL) as input, but this description is less structured and does not facilitate the expression of sequential constraints. This motivates the use of a structured programming language to specify synthesis problems. Transition systems and guarded commands serve as imperative constructs, expressed in a syntax based on that of the modeling language Promela. The syntax allows defining which player controls data and control flow, and separating a program into assumptions and guarantees. These notions are necessary for input to game solvers. The integration of imperative and declarative paradigms allows using the paradigm that is most appropriate for expressing each requirement. The declarative part is expressed in the LTL fragment of generalized reactivity(1), which admits efficient synthesis algorithms, extended with past LTL. The implementation translates Promela to input for the Slugs synthesizer and is written in Python. The AMBA AHB bus case study is revisited and synthesized efficiently, identifying the need to reorder binary decision diagrams during strategy construction, in order to prevent the exponential blowup observed in previous work.

==> eptcsdata.tex <==
\providecommand{\firstpage}{73}
\providecommand{\publicationstatus}{\v{C}ern\'y, Kuncak, Madhusudan (Eds.): Fourth Workshop on\\ Synthesis (SYNT 2015)\\
EPTCS 202, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.202.6}{10.4204/EPTCS.202.6}}
\pdfoutput=1


==> tex/amba.tex <==
\section{Appendix: Supplemental figures}

\begin{figure}
	\centering
	\includesvgpdf[width=\textwidth]{./img/compiler_architecture}
	\caption{
		The compiler architecture that translates \textsc{Promela} source code to a propositional linear temporal logic specification that belongs to the fragment of generalized reactivity of rank 1.}
	\label{fig:compiler_architecture}
\end{figure}

\begin{figure}
	\includesvg[width=\textwidth]{./img/program_to_action_graph}
	\caption{Transformation from a graph whose edges are labeled by program statements, to a graph whose edges are labeled by action formulae $\varphi_{ij}$ (representing each statement) and guards $\hat{varphi}$, derived from the actions using the syntactic approximation of \cref{sec:expressions}.}
	\label{fig:program_to_action_graph}
\end{figure}

\begin{figure}[t]
	\includegraphics[width=0.4\textwidth]{action_expression.pdf}
		\hspace{1cm}
	\includegraphics[width=0.4\textwidth]{action_guard.pdf}
	\caption{The syntactic approximation that defines guards for actions, i.e., for expressions that contain primed variables.
	The left syntax tree corresponds to the action formula $a \wedge \neg a' \wedge \left(b \vee (c \leq 1)\right) \wedge b' \wedge \neg d' \wedge (2 < c')$ and the right syntax tree corresponds to its guard $a \wedge \neg a' \wedge c$, where $a$ is a propositional environment variable, $, b, d$ are propositional system variables, and $c$ and integer system variable.}
	\label{fig:syntactic-approximation}
\end{figure}

\begin{figure}
	\centering
	\includesvg[width=\textwidth]{./img/exclusive_timing_diagram}
	\caption{Timing diagram of atomic execution for a system process with \texttt{gid} $j$.
		The variables $x$ are controlled by other processes and $y$ by the atomically executing system process.
		The variables $x$ “freeze” ($x_{n+1}' = x_{n+1}$) after atomic execution starts at time $n$.
		In addition, the formula $\psi_{\mathrm{masked} }$ deactivates a safety assertion $\phi$ that was defined in an assertion \texttt{ltl} block, so that it won't observe any intermediate states produced during atomic execution.}
	\label{fig:exclusive_timing_diagram}
\end{figure}


\section{Appendix: AMBA AHB Case study}

Declarative specifications for this case study were presented in \cite{Bloem07date,Bloem07cocv,Bloem12jcss,Godhal13sttt}.
These papers do not mention the processors used as hardware, so the difference in processor clock speed is unknown.
As a result, the speedups can be compared only as absolute time intervals.

We base our specifications on those of \cite{Bloem12jcss}.
In that case study, each requirement was obtained either:
\begin{itemize}
	\item by formalizing the AMBA AHB standard, or
	\item by adding some desired (e.g., fair arbiter) or auxiliary properties (e.g., auxiliary scheduling variables \texttt{start}, \texttt{decide}), that are left unspecified in the standard.
\end{itemize}

When initially formalized in LTL, some of the requirements yield formulae that are not in the GR(1) fragment.
Nonetheless, there do exist deterministic B\"{u}chi automata for these particular properties.
The next step in \cite{Bloem12jcss} is to translate these properties to (symbolic) deterministic B\"{u}chi automata, whose states are represented by auxiliary variables that become part of the problem's alphabet.
This translation is not always trivial.

The translation step can be done either manually or automatically.
%
However, with automatic translation the user has little control over the form of the determinized automaton.
This ability to modify the automaton itself proves important during development and, especially, while debugging the specification.
By changing directly the automaton, one can observe what effects small modifications have on realizability, and understand better the problem's structure.

Another aspect of writing LTL formulae, instead of attempting to express the design intent as an automaton, is that the former may require nesting of operators, which quickly becomes unmanageable.
Writing imperatively a B\"{u}chi automaton for the same property can prove easier.
Moreover, as the reduction of progress conditions in the AMBA example demonstrates, the availability of imperative elements can {\em encourage} modifications that significantly reduce the problem's complexity, while preserving the required property.

For this reason, describing directly automata can benefit the synthesis process.



\def\HMASTLOCK{\mathit{HMASTLOCK}}
\def\HBURST{\mathit{HBURST}}
\def\INCR{\mathit{INCR}}
\def\HBUSREQ{\mathit{HBUSREQ}}
\def\HLOCK{\mathit{HLOCK}}
\def\HMASTER{\mathit{HMASTER}}
\def\HGRANT{\mathit{HGRANT}}

The properties from \cite{Bloem12jcss} have been either:
\begin{itemize}
	\item changed, because they did not correspond to the ARM standard, or
	\item expressed {\em directly} as automata, in case they do not belong to GR(1) (similarly to what was done in \cite{Bloem12jcss} by defining the automata directly in LTL), or
	\item equivalently expressed as automata, because this allows significant reduction in synthesis time, or
	\item reformulated to an equivalent, but syntactically simpler formula, in several cases due to the availability of array arithmetic, or
	\item remained unchanged.
\end{itemize}
The correspondence is noted inline, for example, “G 5” is the guarantee with index 5 in \cite{Bloem12jcss}.
In what follows, we consider each specification in incremental order, using the numbering in \cite{Bloem12jcss}.
%
Also, note that a Mealy game is solved here, whereas a Moore game is solved in \cite{Bloem12jcss}.


\subsection{A1 vs ARM standard}

Consider A1, stating that for locked indefinite duration bursts, the master that controls the bus must eventually withdraw its request for {\em access} to the bus.
In logic, this property is expressed as:
\myeq{
	\always \Big( \big(\HMASTLOCK \wedge (\HBURST = \INCR)\big) \rightarrow
		\\
	\nxt \eventually \neg \HBUSREQ[\HMASTER] \Big)
}
The ARM standard states that:
\begin{itemize}
	\item Sec.3.11.2, paragraph 2, p.3-29 and Sec. 3.11.4, p.3-33: A master can lose ownership of the bus early, because the arbiter decides to limit their access time.
	\item Sec.3.11.2, paragraph 3, p.3-29 and Sec. 3.11.5, p.3-34: If a master requests both:
	\begin{enumerate}
		\item bus access (by setting $\HBUSREQ[i]$ HIGH), and
		\item locking of its access (by setting $\HLOCK[i]$ HIGH)
	\end{enumerate}
	then: if the arbiter decides to give to the master the bus, {\em and} lock the access,
	then the arbiter guarantees that it will maintain the lock,
	\begin{quotation}
		“until the {\em locked sequence} has completed”.
	\end{quotation}
\end{itemize}
The question becomes what completion of a locked sequence means.
If a sequence has predefined length (determined by $\HBURST$ and some other signals), then the arbiter knows how long the request will last (G3 addresses this for length-4 locked bursts).

However, for indefinite length bursts, the arbiter does not know a priori when the locked sequence will terminate.
In \cite{Bloem12jcss}, the “locked sequence” is interpreted as the time interval until the master who was granted locked access stops requesting bus {\em access}.
The master withdraws its request for access by setting $\HBUSREQ[\HMASTER]$ to false.
%
As a consequence, the progress assumption A1 requires that a master who requested indefinite locked access, eventually withdraw its request to communicate.


However, it is not clear from the standard whether this behavior is intended.
In Table 2-2, entry $\HLOCK$, p.2-5, it is stated that

\begin{quotation}
	“When HIGH, this signal indicates that the master requires locked access to the bus, and no other master should be granted the bus {\em until} this signal is LOW.”
\end{quotation}
The “until” above suggests that the arbiter {\em can} grant the bus to {\em another} master, {\em after} master $j$ deasserts the signal $\HLOCK[j]$.
This implies that deassertion of $\HLOCK[j]$ by the current master suffices to allow the arbiter to reassign the bus.
It does not refer to the signal $\HBUSREQ[j]$.


\subsection{Weakening A1}

Based on the previous note, we can arrive at a weaker assumption, that decouples the:
\begin{enumerate}
	\item lock requests $\HLOCK$, from the
	\item bus access requests $\HBUSREQ$.
\end{enumerate}
As soon as a master withdraw its request for locking its access, the arbiter is allowed to assign the bus to another master.
This does not oblige the current master to withdraw its request for bus access.
So the master is free to keep requesting bus access ($\HBUSREQ$), but is obliged to stop requesting the lock ($\HLOCK$).
In other words, a master is not allowed to lock the bus forever (but may keep requesting bus access forever, without ever lowering $\HBUSREQ[j]$, in agreement with Sec. 3.11.2, paragraph 1, p.3-29 “A bus master \dots may request the bus during any cycle”).

The new assumption A1 is
\myeq{
	\always (
	(
		\HMASTLOCK \wedge (\HBURST = \INCR)
	)
		\rightarrow
	\nxt \eventually \neg \HLOCK[\HMASTER]
	)
}
We will remove also $(\HBURST = \INCR)$, for reasons explained later.

Note that up to here, this allows the master to stop requesting bus access (LOW $\HBUSREQ$), but keep requesting the lock (during an indefinite length burst).
Sec 3.11.2, paragraph 6, p.3-29 assumes that the master never does this.
It is formulated as assumption A3.
As commented later, we remove assumption A3, because it is not necessary for realizability (and simplifying it has no adverse effect -- weakening of assumptions is desirable).


\subsection{Updating G2}

The replacement of $\HBUSREQ[\HMASTER]$ by $\HLOCK[\HMASTER]$ in A1 implies that the same replacement applies to G2 also.


\subsection{A3 becomes trivially true}

The replacement of $\HBUSREQ[\HMASTER]$ by $\HLOCK[\HMASTER]$ in A1 allows each master $i$ to keep $\HBUSREQ[i]$ always HIGH.
As a result, assumption A3 does not constrain the environment in a way essential for realizability (since the environment can set HIGH all the elements of array $\HBUSREQ$ forever).
Therefore, we drop assumption A3.


\subsection{Coupling between A1 and G2}

\subsubsection{Coupling}

In this section, we analyze the dependence of G2 on A1.
The conclusion motivates simplifying A1.

An initial (wrong) attempt to express the LTL property A1 in \textsc{Promela} (without using Fig.9(a) \cite{Bloem12jcss}) resulted in the code
\begin{verbatim}
assume active env proctype withdraw_lock(){
    progress:
    do
    :: lock && (burst == INCR);
        do
        :: ! master_lockreq; break
        :: true /* wait */
        od
    :: else
    od
}
\end{verbatim}
We have used \verb+master_lockreq+ in place of $\HMASTLOCK[\HMASTER]$, for reasons explained later.

The correct automaton for property A1 is Fig.9(a), and is expressed by the code
\begin{verbatim}
assume active env proctype withdraw_lock(){
progress0:
    do
    :: lock && (burst == INCR); goto S1;
    :: else
    od;
    S1:
    do
    :: (! master_lockreq) && ! (lock && (burst == INCR));
        goto progress0
    :: (! master_lockreq) && (lock && (burst == INCR));
        goto progress1
    :: else
    od;
    progress1:
    do
    :: master_lockreq; goto S1;
    :: (! master_lockreq) && (lock && (burst == INCR));
    :: else;
        goto progress0
    od
}
\end{verbatim}

The specification with the first automaton as A1 is unrealizable.
Using the second automaton, the specification is realizable.

Consider the first automaton and the automaton for G2:
\begin{verbatim}
assert active sys proctype maintain_lock(){
    do
    :: lock && start && (burst == INCR);
        do
        :: ! start && ! master_lockreq; break
        :: ! start
        od
    :: else
    od
}
\end{verbatim}
Each of them has two states: an “initial” one (outer \texttt{do}), and a “waiting” one (inner \texttt{do}).
The product of the two automata has 4 states:

State 0: both automata at the initial states.
The system has not yet lost at this state.

State 1: both automata at the “waiting” states.
As soon as the environment sets \verb+master_lockreq+, the system returns to the initial state and is released, so that it can start a new bus access later.
(The environment also returns to its initial state).

State 2: the environment at the initial state, and the system at the waiting state.
The system has lost, because the initial A1 state is a progress state, and the environment can keep $\HBURST$ different from $\INCR$, to remain at its initial state.
So the environment is not obliged to withdraw the lock request \verb+master_lockreq+, leaving the system indefinitely trapped at its waiting state.

State 3: the system at the initial state, and the environment at its waiting state.
Note that state 3 is reachable, because the environment can reach its waiting state as soon as \verb+lock && (burst == INCR)+, whereas the system has to wait until \verb+start+, and \verb+start+ can be delayed arbitrarily long by the environment keeping \verb+ready+ LOW (G1).

If the system transitions to its waiting state, but the environment remains at its waiting state, then state 1 is reached.
%
If the environment transitions to its initial state, but the system remains at its initial state, then state 0 is reached.
%
These two transitions cause no problems.

The transition that makes the system lose is if the environment returns to its initial state, and the system transitions to its waiting state, both at the same time.
If this happens, then state 2 is reached, and the system has lost.
This transition is possible, only if \verb+burst == INCR+ can hold when \verb+! master_req+.

This execution is not possible with the automaton of Fig.9(a), because in order for the environment to return to \texttt{progress0} there, it must set both \verb+burst != INCR+ {\em and} \verb+! master_req+ at the same time.
This implies that the environment will return to its initial state, without letting the system transition from its initial, to its waiting state.
So it prevents the transition from state 3 to the losing state 1.


\subsubsection{Modifying A1 to remove the coupling}

The coupling analyzed previously requires that the original automaton be used for assumption A1 (which can be rewritten, using structured programming constructs).
The resulting specification is more fragile (for example, the initial attempt at manually writing an automaton contained the error above).
Moreover, it results in longer synthesis time.

For these reasons, we simplify assumption A1 to
\myeq{
	\always (\HMASTLOCK \rightarrow \nxt \eventually \neg \HLOCK[\HMASTER])
}
Using the replacement bit variable \verb+! master_req+, this is equivalent to the (much simpler) automaton
\begin{verbatim}
assume active env proctype withdraw_lock(){
    progress:
    do
    :: lock;
        do
        :: ! master_lockreq; break
        :: true /* wait */
        od
    :: else
    od
}
\end{verbatim}
Note that the only modification from the erroneous initial attempt is to remove the conjunct \verb+burst == INCR+ from the guard \verb+lock && (burst == INCR)+.

The modified assumption A1 states that if the current master is granted the lock, then next it must eventually withdraw the locking request.
This assumption is reasonable, because no master that has been granted locked bus access is entitled to continue requesting the lock indefinitely.
Moreover, it decouples the type of burst from the lock requests.


\subsection{Reducing the number of variables modeling the environment}


\subsubsection{Substitutions}

Earlier, we used \verb+master_lockreq+ in place of $\HLOCK[\HMASTER]$.
The reason is that assumption A3 does not constrain $\HLOCK$ any more (and was dropped, as explained earlier), so each bit in the array $\HLOCK$ can take any value in its domain (no constraint).
Therefore, it is not significant {\em which} bit this is, so $\HMASTER$ can be removed, abstracting the value $\HLOCK[\HMASTER]$ by a single environment bit \verb+master_lockreq+.

This implies the same replacement, of $\HLOCK[\HMASTER]$ by the bit \verb+master_lockreq+, also in G2.

The only remaining use of array $\HLOCK$ is in G7.
Using arrays, the guarantee G7 can be expressed as
\begin{verbatim}
[] ( decide -> (lockmemo' <-> HLOCK[grant']) )
\end{verbatim}
We observe that \verb+HLOCK[grant']+ above is again an element of the array $\HLOCK$.
Before replacement with bit \verb+master_lockreq+, the only constraint on $\HLOCK$ was A1.
A1 required that $\HLOCK[\HMASTER]$ eventually become LOW, if locked access is granted.

In general, \verb+grant'+ will be a master different than the current (so as to serve all masters), therefore \verb+HLOCK[grant']+ takes values independently of $\HLOCK[\HMASTER]$.
So we abstract \verb+HLOCK[grant']+ by a single environment bit \verb+grantee_lockreq+.
The bit \verb+grantee_lockreq+ represents the lock request of that master that is selected as the next grantee.
The values of \verb+grantee_lockreq+ are not constrained in any way.

The initial condition assumption A4 implies that \verb+master_lockreq+ and \verb+grantee_lockreq+ must be false initially.


\subsubsection{Removing array $\HLOCK$}

The replacements:
\begin{enumerate}
	\item $\HLOCK[\HMASTER]$ by the single bit \verb+master_lockreq+, and of
	\item $\HLOCK[\HGRANT[i]']$ by the single bit \verb+grantee_lockreq+
\end{enumerate}
weaken the assumptions.
Therefore, they are desirable.

After these replacements, the array $\HLOCK$ does not appear in any guarantee or assumption (except the initial condition A4).
Therefore, the array $\HLOCK$ can now be removed.

In the best case ($N=16$ masters), the replacement of the bit array $\HLOCK$ by the 2 bits \verb+master_lockreq+ and \verb+grantee_lockreq+ resulting in a reduction by 16 - 2 = 14 bits.
So it reduces by 28 (14 unprimed and 14 primed copies) the number of environment variables in the binary decision diagram (BDD).
This reduction is significant, because environment variables are universally quantified, leading to an exponential increase in the number of possible next inputs.
This reduction reduced synthesis time.

Instead of 32 possible next environment valuations for $\HLOCK$, this replacement reduces them to 4, so a reduction of universal branching by a factor of 8.



\subsection{Merging progress guarantees}

The second significant change was the merging of the $N$ weak fairness guarantees in G9:
\myeq{
	\bigwedge_{i = 0}^{N - 1} \always \eventually (\HBUSREQ[i] \rightarrow (\HMASTER = i) )
}
into an equivalent B\"{u}chi automaton with a single progress state.
This reduces the $N$ inner fixed point computations in the GR(1) synthesis algorithm, to only a single fixed point computation.
As a result, the number of masters $N$ does not increase any more the number of progress goals that the system must satisfy.

The B\"{u}chi automaton used is
\begin{verbatim}
/* G9: weak fairness */
assert active proctype fairness(){
    int(0, N) count;
    do
    :: ! request[count] || (master == count);
        if
        :: (count < N) && (count' == count + 1)
        :: (count == N) && (count' == 0);
            progress: skip
        fi
    :: else
    od
}
\end{verbatim}
This automaton is {\em equivalent} with the conjunction of weak fairness guarantees, because it
\begin{itemize}
	\item “looks” at each one of them in turn,
	\item waits until that progress requirement is satisfied (\verb+! request[count] || (master == count)+)
	\item then increments the counter \verb+count+ and waits for the next fairness guarantee to be satisfied,
\end{itemize}
until it reaches the last fairness guarantee.
At this point it has completed a round of each fairness guarantee being satisfied, so it visits the progress state, and starts a new round.

The automaton is equivalent to the LTL property
\myeq{
	\always\Bigg(
		\eventually\bigg(
			\Big(\HBUSREQ[0] \rightarrow (\HMASTER = 0) \Big)
			\wedge\\
			\nxt \nxt \eventually \Big(
				\big(\HBUSREQ[1] \rightarrow (\HMASTER = 1) \big)
				\wedge
				\dots
			\Big)
		\bigg)
	\Bigg)
}

This demonstrates the merits of using a language that allows directly writing sequential composition.
The result allowed synthesizing arbiters for up to 16 masters, when the previously possible number was 12 (with the specification from \cite{Bloem07cocv}).

Note that this automaton does {\em not} constrain in any way the order in which the arbiter chooses masters to grant the bus.
In other words, it does not restrict the master to using a particular priority for choosing masters.

Note that, after all these changes, the result is a fully parameterized program, where one need only change a single preprocessor definition (\verb+#define N 15+), in order to define a different number of masters in the bus.

\subsection{Changes to variables}

Note that we use an integer variable to model the $HGRANT$ signal.
This conforms to the standard, because the standard requires that exactly one $HGRANT_i$ bit be true at a time.
So we reduce the number of BDD variables by a factor exponential in the number of masters.
The synthesized integer values of $HGRANT_i$ can readily be mapped to patterns of 7 bits, where only a single one is true.


\section{Appendix: Note on deterministic automata}

Note that the (symbolic) automaton is deterministic, because it commits to the choices it makes, i.e., its existential branching is visible to the property (the variables that represent the state are letters in the alphabet).
(For automated determinization of LTL properties to either parity or B\"{u}chi automata, prior to solving a parity game, see \cite{Sohail08vmcai}).

For example, an automaton with four nodes can be represented by introducing an auxiliary integer variable $u \in \{0, 1, 2, 3\}$.
Suppose that it has the transitions
$
	( (u = 0) \rightarrow (
		( \varphi_1 \wedge \nxt (u = 1) ) \vee
		( \neg \varphi_1 \wedge \nxt (u = 0) )
	) )
		\wedge
	( (u = 1) \rightarrow (
		( \varphi_2 \wedge \nxt (u = 2) ) \vee
		( \varphi_3 \wedge \nxt (u = 2) )
	) )
		\wedge
	( (u = 2) \rightarrow (
		( \varphi_4 \wedge \nxt (u = 3) ) \vee
		( \varphi_5 \wedge \nxt (u = 2) ) \vee
		( \neg \varphi_4 \wedge \neg \varphi_5 \wedge \nxt (u = 2) )
	) )
		\wedge
	( (u = 3) \rightarrow (\varphi_6 \wedge \nxt (u = 0) )
$.
It can be argued that this formula is much less readable and editable than the listing of \cref{fig:formula-as-listing}.
\begin{figure}
	\centering
\begin{minipage}[b]{3cm}
\begin{lstlisting}
do
:: $\varphi_1$;
	if
	:: $\varphi_2$
	:: $\varphi_3$
	fi
	do
	:: $\varphi_4$; break
	:: $\varphi_5$;
	:: else
	od
	$\varphi_6$
:: else
od
\end{lstlisting}
\end{minipage}
\caption{Listing corresponding to formula in text.}
\label{fig:formula-as-listing}
\end{figure}

Note that the above automaton can have more than a single enabled transition.
It is still a deterministic Buchi automaton, because the program counter $u$ is visible to the environment.
This forces the system to commit to its future strategy during GR(1) synthesis, when it selects a valuation of its variables as reaction.
In other words, the non-determinism is visible, because $u$ is part of the alphabet and so of the moves that the synthesis algorithm takes in the game.
%
For the above symbolic automaton to be non-deterministic, the variable $u$ must not be part of the alphabet, so not a visible output.
This is not the case in GR(1) synthesis.


==> tex/preamble.tex <==
\RequirePackage{snapshot}
\setcounter{tocdepth}{3}
\usepackage{amsmath,amssymb}
\usepackage{graphicx,subcaption,wrapfig}
\captionsetup{compatibility=false}
\graphicspath{{./img/}}
\usepackage{listings,color,multicol,verbatim,url,textcomp}
\usepackage{booktabs,array,multirow,multicol}
\usepackage{mycommands,formal_methods_commands}
\newcommand{\keywords}[1]{\par\addvspace\baselineskip
\noindent\keywordname\enspace\ignorespaces#1}

\pdfmapfile{+ltlfonts.map}

\renewcommand\topfraction{0.85}
\renewcommand\bottomfraction{0.85}
\renewcommand\textfraction{0.1}
\renewcommand\floatpagefraction{0.85}

\def\tla@while{-\hspace{-.18em}\triangleright}
\def\tlawhilep{\stackrel{\mbox{\raisebox{-.3em}[0pt][0pt]{$\scriptscriptstyle+\;\,$}}}{\tla@while}}

\def\strictarrow{\stackrel{\mbox{\raisebox{-.3em}[0pt][0pt]{$\scriptscriptstyle\mathrm{sr}\;\,$}}}{\tla@while}}

\definecolor{deepblue}{rgb}{0,0,0.5}
% \newfontfamily{\couriernew}{Courier New}
\lstset{%
	language=Promela,%
	basicstyle=\ttfamily\scriptsize,%
	numbers=left,%
	stepnumber=1,%
	numbersep=5pt,%
	keywordstyle=\color{deepblue},%
	commentstyle=\color[rgb]{0.133,0.545,0.133},%
	stringstyle=\color{deepgreen},%
	showstringspaces=false% 
	captionpos=b,%
	breaklines=true,%
	breakatwhitespace=false,%
	mathescape,
	frame=single,
	morekeywords={assume,env,sys,free,ltl,sync,async}}%

% top matter
\author{Ioannis Filippidis \qquad Richard M. Murray
\email{\{ifilippi, murray\}@caltech.edu}
\institute{Control~and~Dynamical~Systems,\\
California~Institute~of~Technology,\\
Pasadena~CA~91125, USA}
\and
Gerard J. Holzmann
\email{gerard.j.holzmann@jpl.nasa.gov}
\institute{Laboratory~for~Reliable~Software,\\
Jet~Propulsion~Lab, Caltech,\\
Pasadena~CA~91109, USA}
}
\def\authorrunning{I. Filippidis, R.M. Murray, G.J. Holzmann}

\title{A multi-paradigm language for reactive synthesis}
\def\titlerunning{A multi-paradigm language for reactive synthesis}

